Leveraging Augmented Reality for Improved Situational Awareness During UAV-Driven Search and Rescue Missions

In the high-stakes domain of search-and-rescue missions, the deployment of Unmanned Aerial Vehicles (UAVs) has become increasingly pivotal. These missions require seamless, real-time communication among diverse roles within response teams, particularly between Remote Operators (ROs) and On-Site Operators (OSOs). Traditionally, ROs and OSOs have relied on radio communication to exchange critical information, such as the geolocation of victims, hazardous areas, and points of interest. However, radio communication lacks information visualization, suffers from noise, and requires mental effort to interpret information, leading to miscommunications and misunderstandings. To address these challenges, this paper presents VizCom-AR, an Augmented Reality system designed to facilitate visual communication between ROs and OSOs and their situational awareness during UAV-driven search-and-rescue missions. Our experiments, focus group sessions with police officers, and field study showed that VizCom-AR enhances spatial awareness of both ROs and OSOs, facilitate geolocation information exchange, and effectively complement existing communication tools in UAV-driven emergency response missions. Overall, VizCom-AR offers a fundamental framework for designing Augmented Reality systems for large scale UAV-driven rescue missions.

==> parking-lot/evaluation2.tex <==


% \textbf{RQ2:How does the system compare to radio communication for communicating geolocation information}

% We have extended the above framework and developed a new system(VizCom-AR) to test how effective our approach is when compared to Radio for communicating geolocation information.


% \label{sec:framework}


% This feedback loop is crucial for ROs to maintain situational awareness and to coordinate the next steps effectively.  In this way, \system supports bi-directional visual communication between ROs and OSOs. Since \system is capable of computing and persisting the geolocation of POIs, semi-autonomous UAVs can utilize this information for decision-making and flight planning activities. It is important to note that this aspect of the system is beyond the scope of this research article. In summary, \system enables the sharing of key mission information among all mission participants, including UAVs. This exchange of information is done in a format that enhances comprehension and facilitates coordinated actions. Figure \ref{fig:s1} illustrates the relationship between various components of \System. We now describe the design of each interface, \Dronear, and \humanar in complete detail. 

% \footnote{Demo Videos: \url{https://www.youtube.com/playlist?list=PLU5_FMa4WPVgTSWHJmmdHVK-Eu3HvZLRS}}
% The \dronear and \humanar  are standalone Location-Based Augmented Reality applications developed in the Unity \cite{Unity:online} environment using ARKit \cite{AR-kit:online} platform. We study the usability of our interfaces for supporting collaboration between ROs and OSOs, the applicablity of the overall \system in the real-world, and explore future system design opportunities in the domain of UAV-driven emergency response missions.



% \begin{figure}[htbp]
%   \centering
%   \subfloat[The user specifies the POI (Injured Person) by marking the area of the screen with an appropriate symbol on the aerial video stream of UAV-1 via \dronear. \system computes the geolocation of the point of interest and uses it to augment the aerial video stream with the symbol. ]{\includegraphics[width=0.45\columnwidth]{figures/drone-ar/drone-ar-ipad.png}
%   \label{fig:remote-team-interface-drone-1}}
%   \hfill
%   \subfloat[The system persists the geolocation of the POI (Injured Person) identified in the aerial video stream of the UAV-1. Therefore, \dronear uses it to augment the video stream of UAV-2 in the same mission with an appropriate marker when its camera looks towards the POI's geolocation.  ]{\includegraphics[width=0.45\columnwidth]{figures/drone-ar/drone-2-ar-ipad-new.png}
%   \label{fig:remote-team-interface-drone-2}}
%   \caption{POI annotation and visualization over aerial video streams of multiple UAVs via \dronear interface}
% \end{figure}



% \ankit{Maybe out of scope now}
% \subsubsection{Multi-UAV POI Visualization} 
% To preserve the geolocation information in a way that can be shared with other UAVs participating in the mission, all symbols corresponding to POIs are persisted in the AR world space of \dronear based on their geolocation. In our implementation, all UAVs are part of a single AR world space. Therefore, POIs added from different UAVs persist in this common AR space, allowing each UAV to share and augment POIs in their aerial video streams based on their own location and their captured field of view in the AR World Space. To support the POI visualization for multi-UAV emergency response missions, we leverage the AR world tracking feature of the ARKit platform to render the POI annotated in the aerial video stream of one UAV into the aerial video stream of other UAVs participating in the same mission. Figures \ref{fig:remote-team-interface-drone-1} and  \ref{fig:remote-team-interface-drone-2} illustrate the multi-UAV POI visualization whilst searching for an injured person. The sequence of events for multi-UAV POI visualization is as follows; first, the victim is detected in the aerial video stream of a UAV (e.g., UAV-1, Figure \ref{fig:remote-team-interface-drone-1}) and a user marks the victim on the video stream; second, \system computes the geolocation of the injured person and stores it in the shared AR space. Finally, the AR cameras of other UAVs (e.g., UAV-2, Figure \ref{fig:remote-team-interface-drone-2}) track the same AR World Space and render the POI overlay into their own video streams when the POI appears within their camera's field of view. 

% % \reviewer{As the reader, I would like to know how the authors accurately established and maintained a shared AR world space of multiple UAVs operating in the field. } \ankit{added a figure to make it very intuitive now}






% Additionally, \humanar leverages web-socket connections over Wi-Fi and LTE channels to exchange data such as geolocation of POIs with other emergency response tools. Hence, the extensible design of \humanar allows it to receive GPS locations of POI at run-time from UAVs, \dronear, and can work in conjunction with other emergency rescue tools.


% We implemented \humanar as an AR System using Unity Platform, for Microsoft Hololens 2 \cite{Microsof61:online}. \humanar creates its own AR World Space, where a single AR camera tracks and mimics the position, orientation, and camera properties such as Field-of-View of the OSO's AR Headset in the real world. POIs in the AR world space of \humanar are added through the Real-Time cloud database component of \system via a secure Wi-Fi channel. During the mission, after an RO adds a POI using \dronear, the real-time database of \system receives the essential POI details such as its type, geolocation, and other metadata necessary for unique identification. To synchronize \humanar's AR world space with all POIs, \humanar sends web requests to the real-time database to fetch data every 5 seconds. We poll POI data at this interval to keep network traffic low. This strategy allows \humanar to dynamically add any number of POIs based on the geolocation information received from the real-time database for OSO visualization. Similarly, data from \humanar, such as the OSO's location or the next POI they plan to visit, is sent to \dronear via the real-time cloud database. This enables the RO to visualize information on the Aerial Video Stream and monitor the OSO's mission progress. Figure \ref{fig:firstresponse-ar-implementation} shows a block diagram illustrating the information flow between the \humanar and \dronear interfaces.





==> sections/analysis.tex <==
\section{Analysis}

For this study, data was meticulously gathered using a Parrot ANAFI drone. The drone operations were automated and controlled through a script, ensuring consistency and accuracy in data collection. This approach allowed for the precise manipulation of the drone's altitude, pitch angles, and velocities as per the requirements of the study.

We collected data at three different altitudes: 10 meters, 20 meters, and 30 meters, chosen to provide varied perspectives from close to moderately elevated heights. Alongside altitude, the drone was maneuvered at four pitch angles: 45, 60, 75, and 90 degrees, each offering a unique orientation relative to the ground. To assess the algorithm's adaptability to different speeds, the drone was flown at velocities of 5 meters per second, 10 meters per second, and 15 meters per second. This range encompassed slow, stable flight to faster, more dynamic movement. We captured videos along with corresponding metadata for each combination of altitude, pitch angle, and velocity. 

During the data collection phase, we strategically positioned a 3ft x 4ft whiteboard in a green field. This setup facilitated the capture of video data, essential for our analysis. The placement of the whiteboard was particularly crucial, as it enabled us to detect the board using OpenCV contour detection techniques accurately. This detection process allowed us to obtain the precise pixel coordinates of the target. Additionally, we manually calculated the GPS location of the whiteboard using Google Maps, which served as the ground truth value in our study.


\textbf{Accuracy of Geolocation computation.}

Initially, we processed the collected video data by extracting frames from each video. Our focus was on selecting frames that represented various instances when the Point of Interest (POI) appeared in different locations on the screen. To ensure comprehensive coverage and variability, we selected 10 frames for each unique position combination.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/analysis/Geolocation Computation/Altitude_violin.png}
    \caption{GeoLocation Computation Accuracy }
    \label{fig:distance-altitude}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/analysis/Geolocation Computation/Pitch_violin.png}
    \caption{GeoLocation Computation Accuracy }
    \label{fig:distance-pitch}
\end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/analysis/Geolocation Computation/Velocity.png}
%     \caption{GeoLocation Computation Accuracy }
%     \label{fig:flying-ar-implementation}
% \end{figure}
In the selected frames, we employed OpenCV contour detection to identify the middle point of the whiteboard. To minimize errors and enhance accuracy, our approach involved considering only those contours that exceeded a predefined area threshold. This method effectively eliminated smaller dots that were otherwise erroneously detected as false positives. After the contour detection, each frame underwent a manual review. This review process was pivotal in verifying the accuracy of the detected middle points and making necessary corrections where discrepancies were found.


Following the successful identification of the whiteboard's middle point in each frame, we processed the frame's metadata. This metadata was then utilized as a critical input for our geolocation calculation algorithm. Through this process, we ensured that the geolocation data was both accurate and relevant to the specific context of each frame.

\textbf{Results:}
We calculated the geolocation of the whiteboard(POI) for all the data collected above and plotted the geolocation accuracy across different Altitudes and Pitch Angles.
There are no useful insights for velocity as we are calculating geolocation for a frame.

 
We used the distance(Geodesic distance) between the calculated and measured coordinates of the target object to estimate the horizontal accuracy of our computed geolocations.
Figure \ref{fig:distance-altitude} shows the mean horizontal accuracy of the calculated geolocations of the target object across various altitudes. Accuracy decreased as altitude of the UAV increased. Mean accuracy at 10m, 20m, and 30m altitudes are 1.3 meters, 2.5 meters, and 2.9 meters

Figure \ref{fig:distance-pitch} shows the mean horizontal accuracy of the calculated geolocations of the target object across various camera pitch angles. Accuracy decreased as the camera pitch angle decreased. Accuracy is highest when camera is looking perpendicular to the ground. Mean accuracy at 45,60,75 and 90 pitch angles are 3.6m, 2.2m, 1.8m, and 1.5m.



\textbf{Accuracy of object augmentation.}

Our analysis is centered on evaluating the accuracy of the augmented marker in the Unity AR space. Each video from our dataset was streamed to the Unity application, where the measured location of the whiteboard served as the Point of Interest (POI). In Unity, a marker was augmented to represent the whiteboard's position. Frames are extracted for each video using the Unity screen recorder during the stream.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/analysis/Marker Augmentation/Altitude_violin.png}
    \caption{Marker Augmentation Accuracy }
    \label{fig:pixelDistance-altitude}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/analysis/Marker Augmentation/Pitch_violin.png}
    \caption{Marker Augmentation Accuracy }
    \label{fig:pixelDistance-pitch}
\end{figure}

Similar to the computation of geolocation accuracy, we extracted 10 frames from each combination collected during our data collection phase. Within each frame, there are two distinct white objects: one representing the augmented Point of Interest (POI) and the other being the whiteboard itself. We utilized contour detection to determine the midpoints of both these white objects, in instances of overlap between the two objects, contour detection identified only a single contour. In such cases, we considered the midpoint of this single detected contour as the representative midpoint for both objects. After identifying the midpoints of the two white objects in each frame, we proceeded to calculate the Euclidean distance between these midpoints. This calculation was performed for every frame, providing a quantitative measure of the pixel distance between the augmented Point of Interest (POI) and the actual whiteboard. The Euclidean distance served as a crucial metric for assessing the precision of our augmented reality overlay compared to the physical location of the whiteboard in the video stream. 



\textbf{Results:}
Figure \ref{fig:pixelDistance-altitude} shows the mean pixel distance between the augmented marker and whiteboard across various altitudes. Pixel distance of the augmented object is more when the altitude is low as we are closer to the ground and UAVs FOV is covering less area. At 10m altitude, there are more overlaps of marker and whiteboard. 

Figure \ref{fig:pixelDistance-pitch} shows the mean pixel distance between the augmented marker and whiteboard across various camera pitch angles. Accuracy decreased as the camera pitch angle decreased. Similar to geolocation computation accuracy, marker augmentation accuracy decreases as the pitch angle is decreased and is highest when the camera is looking perpendicular to the ground.


\textbf{Performance analysis for Multi-UAV }

This section offers an in-depth examination of the system’s performance characteristics, with a specific focus on the scaling behavior of the Unity application as multiple UAVs are added. This analysis aims to understand how the addition of UAVs impacts overall system performance, latency, and resource utilization. Specifications of the system used for the test are shown in Table \ref{table:specs}. We have conducted a comparison of the CPU and memory utilization while the application is operational. Notably, the usage of the GPU remains at zero. Figure \ref{fig:performance-cpu} illustrates the increase in CPU usage as the system expands from 1 to 12 UAVs. As the number of UAVs grows, there is a corresponding rise in CPU utilization. Likewise, Figure \ref{fig:performance-memory} demonstrates that memory usage also escalates with the addition of more UAVs. The system crashed during a test with 12 UAVs as a result of memory resources being fully exhausted, leading to a state of 100 percent memory utilization.

\begin{table}[h!]
\centering
\caption{System Specifications}
\begin{tabular}{|p{2.5cm}|p{7cm}|}
\hline
\textbf{Specification} & \textbf{Details} \\
\hline
Hardware Model & Dell Inc. Precision 3460 \\
\hline
Memory & 16.0 GiB \\
\hline
Processor & 12th Gen Intel\textregistered Core\texttrademark i7-12700 x 20 \\
\hline
Graphics & NVIDIA Corporation TU117GLM [Quadro T1000 Mobile] \newline Mesa Intel\textregistered UHD Graphics 770 (ADL-S GT1) \\
\hline
Disk Capacity & 512.1 GB \\
\hline
OS Name & Ubuntu 22.04.3 LTS \\
\hline
OS Type & 64-bit \\
\hline

\end{tabular}

\label{table:specs}
\end{table}




\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/analysis/performance_analysis/CPU_new.png}
    \caption{CPU Utilization }
    \label{fig:performance-cpu}
\end{figure}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/analysis/performance_analysis/memory_new.png}
    \caption{Memory Utilization }
    \label{fig:performance-memory}
\end{figure}



==> tables/survey_results.tex <==

\begin{table}[htbp]
    \centering
    \begin{tabular}{|c|m{37em}|c|}  
    \hline
    \textbf{Qs} & \textbf{Statement} & Average Rating\\ 
	\hline
	Q1 & I believe the system's ability to geolocate POIs could benefit the police officers in carrying out their investigations & 5\\
	\hline
	Q2 & I believe that visualizing the POIs using AR Glasses can assist on-scene officers in quickly assessing the situations & 4.8\\
	\hline
	Q3 & The system could support police officers in sharing and understanding the geolocation information during emergency response & 4.2\\
	\hline
	Q4 & The system could be a valuable addition to our existing communication system & 4.2 \\
	\hline
	
	
\end{tabular}
    \caption{Detailed description of the statements included in the survey questionnaire for police officers}
	\label{tab:survey_questions}
\end{table}
